The Reactor: A fast and sample-efficient Actor-Critic agent for Reinforcement Learning

In this work we present a new agent architecture, called Reactor, which combines multiple algorithmic and architectural contributions to produce an agent with higher sample-efficiency than Prioritized Dueling DQN (Wang et al., 2016) and Categorical DQN (Bellemare et al., 2017), while giving better run-time performance than A3C (Mnih et al., 2016). Our first contribution is a new policy evaluation algorithm called Distributional Retrace, which brings multi-step off-policy updates to the distributional reinforcement learning setting. The same approach can be used to convert several classes of multi-step policy evaluation algorithms designed for expected value evaluation into distributional ones. Next, we introduce the \b{eta}-leave-one-out policy gradient algorithm which improves the trade-off between variance and bias by using action values as a baseline. Our final algorithmic contribution is a new prioritized replay algorithm for sequences, which exploits the temporal locality of neighboring observations for more efficient replay prioritization. Using the Atari 2600 benchmarks, we show that each of these innovations contribute to both the sample efficiency and final agent performance. Finally, we demonstrate that Reactor reaches state-of-the-art performance after 200 million frames and less than a day of training.

==> large-noop-summary-table.tex <==
\begin{tabular}{| c | c | c | c |}
\hline
Algorithm & Normalized & Mean& Elo \\
 & scores & rank &\\
\hline
Random & 0.00 & 10.93 & -673\\
Human & 1.00 & 6.89 & 0\\
DQN & 0.79 & 8.65 & -167\\
DDQN & 1.18 & 7.28 & -27\\
Duel & 1.51 & 5.19 & 143\\
Prior & 1.24 & 6.11 & 70\\
Prior. Duel. & 1.72 & 5.44 & 126\\
Rainbow & {\bf 2.31} & 3.63 & 270\\
Reactor ND $^{\ref{reactorfootnote}}$ & 1.80 & 4.53 & 195\\
Reactor & 1.87 & 4.46 & 196\\
Reactor 500m & 2.30 & {\bf 3.47} & {\bf 280}\\
\hline
\end{tabular}


==> summary-table-sparse.tex <==
\begin{tabular}{| c | c c | c | c |}
\hline
Algorithm & \multicolumn{2}{|c|}{Normalized} & Rank & Elo \\
 & \scriptsize{mean} & \scriptsize{median} & \scriptsize{mean} & \\
\hline
Random & 0.00 & 0.00 & 8.86 & -621\\
Human & 1.00 & 1.00 & 2.14 & 0\\
DQN & 0.16 & 0.02 & 7.14 & -461\\
DDQN & 0.14 & 0.00 & 8.57 & -593\\
Duel & 0.03 & 0.00 & 7.29 & -479\\
Prior & 0.18 & 0.01 & 6.29 & -397\\
Prior. Duel. & 0.13 & 0.01 & 8.57 & -593\\
Rainbow & 0.21 & 0.05 & 4.00 & -206\\
Reactor v1 200m & {\bf 0.36} & {\bf 0.30} & {\bf 3.71} & {\bf -179}\\
Reactor v2 200m & 0.32 & 0.12 & 4.71 & -262\\
Reactor v2 500m & 0.33 & 0.19 & 4.86 & -281\\
\hline
\end{tabular}

